An Interpretable X-ray Style Transfer via Trainable Local Laplacian Filter

Radiologists have preferred visual impressions or 'styles' of X-ray images that are manually adjusted to their needs to support their diagnostic performance. In this work, we propose an automatic and interpretable X-ray style transfer by introducing a trainable version of the Local Laplacian Filter (LLF). From the shape of the LLF's optimized remap function, the characteristics of the style transfer can be inferred and reliability of the algorithm can be ensured. Moreover, we enable the LLF to capture complex X-ray style features by replacing the remap function with a Multi-Layer Perceptron (MLP) and adding a trainable normalization layer. We demonstrate the effectiveness of the proposed method by transforming unprocessed mammographic X-ray images into images that match the style of target mammograms and achieve a Structural Similarity Index (SSIM) of 0.94 compared to 0.82 of the baseline LLF style transfer method from Aubry et al.

==> figures/llf_algo_description.tex <==
\begin{algorithm}
\caption{LLF Algorithm}
\label{alg:llf}
\begin{algorithmic}[1]
\State \textbf{Input:} Image $\img \in \mathbb{R}^{M \times N}$
\State Decompose $\img$ into Gaussian pyramid $\mathcal{G}$
\For{each value $\mathrm{p}$ in Gaussian pyramid $\gauss$}
    \State Remap input image:  $ \img' = r(\img - \gp) + \gp$
    \State Compute intermediate Laplacian pyramid $\il$ from $\img'$
    \State Update final Laplacian pyramid: $\Lap(\textrm{p}) = \il(\textrm{p})$
\EndFor
\State Collapse $\Lap$ into output image $\img_{\textrm{out}}$
\State \textbf{Output:} Image $\img_{\textrm{out}} \in \mathbb{R}^{M \times N} $
\end{algorithmic}
\end{algorithm}



==> figures/llf_algorithm.tex <==
\begin{figure*}[tb]
	\centerline{\includegraphics[width=0.6\textwidth]{images/llf_algorithm.pdf}}
	\caption[Local Laplacian Filter Description]{Description of the Local
	Laplacian Filter Algorithm.}
	\label{fig:llf}
\end{figure*}



==> figures/llf_optim.tex <==
\begin{figure*}[tb]
\centering
\includegraphics[width=0.65\textwidth]{images/llf_optim.pdf}
\caption[Optimization of the \ac{llf} with Backpropagation]{This figure depicts 
	the optimization process of the \ac{llf} and the Normalization Layer 
	using backpropagation, along with the matching pairs for the loss 
	function.}

\label{fig:llf_optim}
\end{figure*}



==> figures/remap.tex <==
\begin{figure}[tb]
\centering
\begin{subfigure}{0.38\linewidth}
\includegraphics[width=\linewidth]{images/alpha_remap.pdf}
	\caption{$\remap(x)$ with $ \alpha > 1$}
\label{fig:alpha_remap_suppress}
\end{subfigure}
\hspace{1cm}
\begin{subfigure}{0.38\linewidth}
\includegraphics[width=\linewidth]{images/alpha_remap2.pdf}
\caption{$\remap(x)$ with $ \alpha < 1$}
\label{fig:alpha_remap_enhance}
\end{subfigure}
\begin{subfigure}{0.38\linewidth}
\includegraphics[width=\linewidth]{images/beta_remap2.pdf}
\caption{$\remap(x)$ with $ \beta > 1$}
\label{fig:beta_remap_enhance}
\end{subfigure}
\hspace{1cm}
\begin{subfigure}{0.38\linewidth}
\includegraphics[width=\linewidth]{images/beta_remap.pdf}
	\caption{$\remap(x)$ with $ \beta < 1$}
\label{fig:beta_remap_suppress}
\end{subfigure}

\caption[Local Laplacian Filter Remapping Function]{This figure illustrates the 
	influence of the two parameters, $\alpha$ and $\beta$, on the remapping 
	function, $\remap$. Both parts of $\remap$, namely $\remap_d$ and 
	$\remap_e$, are shown in dark and light blue, respectively.}
\label{fig:remap}

\end{figure}




==> figures/results.tex <==
\newcommand{\llfmapp}{0.20\textwidth}
\newcommand{\llfgap}{0.5pt}
\newcommand{\llfitgap}{14.5pt}

\begin{figure*}[tb]
\centering
	\begin{minipage}{0.8\textwidth}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/data_0.png}
\caption{input}
\end{subfigure}
	\hspace{\llfitgap}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/mlp_with_offset.png}
	\caption{\mlpnorm}
\end{subfigure}
	\hspace{\llfgap}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/mlp_no_offset.png}
	\caption{\mlpremap}
\end{subfigure}

\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/label_0.png}
\caption{target}
\end{subfigure}
	\hspace{\llfitgap}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/classic_remap_with_offset.png}
	\caption{\orignorm}
\end{subfigure}
	\hspace{\llfgap}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/classic_remap_no_offset.png}
	\caption{\orig}
	\label{fig:llf_mapping_orig}
\end{subfigure}
	\hspace{\llfgap}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/gradient_matching.png}
	\caption{\gradientremap}
\label{fig:llf_mapping_gradient}
\end{subfigure}
\end{minipage}



\caption[\ac{llf} Mapped Images with Optimized Remap Functions]{Images mapped 
	using optimized remap functions through \ac{llf}. The display includes 
	gradient matching, \ac{mlp} with and without normalization, and the 
	original remap functions, both with and without normalization layer.}

\label{fig:llf_mapping}

\end{figure*}



==> figures/results_imp.tex <==
\newcommand{\llfmapp}{0.16\textwidth}
\newcommand{\llfgap}{0.5pt}
\newcommand{\llfitgap}{14.5pt}

\begin{figure*}[tb]
\centering

\begin{minipage}[t]{\llfmapp}
\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/data_0.png}
\caption{input}
\end{subfigure}

\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/label_0.png}
\caption{target}
\end{subfigure}
\end{minipage}
\hspace{\llfitgap}
\begin{minipage}[t]{\llfmapp}
\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/mlp_with_offset.png}
	\caption{\ac{mlpnorm}}
\end{subfigure}
\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/mlp_no_offset.png}
	\caption{\ac{mlpremap}}
\end{subfigure}
\end{minipage}
\hspace{\llfgap}
\begin{minipage}[t]{\llfmapp}
\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/classic_remap_with_offset.png}
	\caption{\ac{orignorm}}
\end{subfigure}
\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/classic_remap_no_offset.png}
	\caption{\ac{orig}}
	\label{fig:llf_mapping_orig}
\end{subfigure}

\end{minipage}
\hspace{\llfitgap}
\begin{minipage}[t]{\llfmapp}
\vfill
\begin{subfigure}{\textwidth}
\includegraphics[width=\linewidth]{images/llf_mapping/gradient_matching.png}
	\caption{\ac{gradientremap}}
\label{fig:llf_mapping_gradient}
\end{subfigure}
\vfill

\end{minipage}

\caption{Comparison of \ac{llf}-transformed images against the target image.}
\label{fig:llf_mapping}

\end{figure*}



==> figures/results_imp2.tex <==
\newcommand{\llfmapp}{0.16\textwidth}
\newcommand{\llfgap}{0.5pt}
\newcommand{\llfitgap}{14.5pt}

\begin{figure}[tb]
\centering

\begin{minipage}[t]{\textwidth}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/data_0.png}
\caption{input}
\end{subfigure}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/label_0.png}
\caption{target}
\end{subfigure}
\end{minipage}

\begin{minipage}[t]{\textwidth}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/mlp_with_offset.png}
	\caption{\ac{mlpnorm}}
\end{subfigure}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/mlp_no_offset.png}
	\caption{\ac{mlpremap}}
\end{subfigure}
\end{minipage}

\begin{minipage}[t]{\textwidth}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/classic_remap_with_offset.png}
	\caption{\ac{orignorm}}
\end{subfigure}
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/classic_remap_no_offset.png}
	\caption{\ac{orig}}
	\label{fig:llf_mapping_orig}
\end{subfigure}

\end{minipage}

\begin{minipage}[t]{\textwidth}
\vfill
\begin{subfigure}{\llfmapp}
\includegraphics[width=\linewidth]{images/llf_mapping/gradient_matching.png}
	\caption{\ac{gradientremap}}
\label{fig:llf_mapping_gradient}
\end{subfigure}
\vfill

\end{minipage}

\caption{Comparison of \ac{llf}-transformed images against the target image.}
\label{fig:llf_mapping}

\end{figure}


